A sequential Monte Carlo algorithm for data assimilation problems in ecology

1. Temporal trends in species distributions are necessary for monitoring changes in biodiversity, which aids policymakers and conservationists in making informed decisions. Dynamic species distribution models are often fitted to ecological time series data using Markov Chain Monte Carlo algorithms to produce these temporal trends. However, the fitted models can be time-consuming to produce and run, making it inefficient to refit them as new observations become available. 2. We propose an algorithm that updates model parameters and the latent state distribution (e.g. true occupancy) using the saved information from a previously fitted model. This algorithm capitalises on the strength of importance sampling to generate new posterior samples of interest by updating the model output. The algorithm was validated with simulation studies on linear Gaussian state space models and occupancy models, and we applied the framework to Crested Tits in Switzerland and Yellow Meadow Ants in the UK. 3. We found that models updated with the proposed algorithm captured the true model parameters and latent state values as good as the models refitted to the expanded dataset. Moreover, the updated models were much faster to run and preserved the trajectory of the derived quantities. 4. The proposed approach serves as an alternative to conventional methods for updating state-space models (SSMs), and it is most beneficial when the fitted SSMs have a long run time. Overall, we provide a Monte Carlo algorithm to efficiently update complex models, a key issue in developing biodiversity models and indicators.

==> chuff2.tex <==
\hypertarget{introduction}{%
\section{Introduction}\label{introduction}}

Biodiversity monitoring programs are essential to obtain data for conservation and management decisions. Examples of such monitoring programs include the living planet index dataset \citep{collen2009monitoring}, North American breeding bird survey \citep{bystrak1981north}, record observations of species through time. Ecological time series data can be used to model animal movement
\textbf{{[}citation{]}}, population dynamics \citep{rivot2004bayesian, kery2020applied} etc to make inferences on the changes in biodiversity over time. Information on the distribution in space and time allows for the fitting of dynamic species distribution models (SDMs). These models are scarcely applied in ecology because the spatiotemporal component makes the model computationally intensive because they include many random effects that need to be estimated \citep{dobson2023dynamicsdm, kery2013analysing}, making the dynamic SDMs time-consuming to fit. This issue is exacerbated when species are again observed in the consecutive year after the model has been fitted, and the model parameters need to be updated to reflect potentially rapid changes in species distributions \citep{arulampalam2002tutorial} because the same time-consuming model fitting process needs to be repeated.


We refer to the process of getting new data as data assimilation.

The fitted SDMs can be computationally expensive and may take
longer to run. Since the time series data are sequentially generated (usually
yearly), the SDMs need to be re-fitted when new
streams of data are obtained to reflect the rapid changes in the
distribution of species over time . The latest
data obtained increases the dataset's size which complicates the SDM's
fit and consequently the computation cost of the model.

State-space model (SSM) are SDMs fitted to ecological time series
data. The SSMs are hierarchical models that account for temporal
autocorrelation by providing a model for the state process and another
for the observation process \citep{doucet2001introduction, kery2020applied, auger2020introduction}. The separate state or ecological process model captures
the dynamics of the true underlying state over time and the observation
model describes the stochastic dependence of the observed data on the state
model. The SSMs are used to estimate model parameters, and latent states,
forecast future latent states and observations, the distribution of the
most recent states given the data (filtering distribution of model) and
model likelihood \citep[by integrating over all the latent state dimensions; ][]{newman2023state, durbin2012time}.

SSMs have gained popularity in applied ecology owing to the flexibility in fitting them and availability of packages that provides Monte carlo algorithms (such as for Markov Chain Monte
Carlo (MCMC) and sequential Monte Carlo (SMC)) to fit them \citep{auger2016state}. With the availability of free software for MCMC algorithms such as BUGS \citep{lunn2000winbugs, lunn2009bugs}, JAGS \citep{depaoli2016just}, Stan \citep{carpenter2017stan}, NIMBLE \citep{de2017programming} and many others, ecologist have the freedom to make specifications for the fitted SSMs. 


They are very
flexible especially when Monte Carlo methods such as Markov Chain Monte
Carlo (MCMC) and sequential Monte Carlo (SMC) methods are used to fit them, making
them popular in modelling ecological time series data \citep{auger2016state}. 

The MCMC approach to fitting SSMs has gained popularity in literature \citep{auger2021guide}, especially with the free developed
software for MCMC such as BUGS \citep{lunn2000winbugs, lunn2009bugs}, JAGS \citep{depaoli2016just}, Stan \citep{carpenter2017stan}, NIMBLE \citep{de2017programming} and many others. Although MCMC approaches provide a flexible way to fit SSM, they can be
computationally expensive, and a complex SSM structure can pose
difficulties for model validation and assessment \citep{auger2021guide}. Moreover, the MCMC approach can be slow and sensitive to convergence problems, especially for high-dimensional models and non-linear and non-Gaussian SSMs \citep{wang2007latent, peters2010ecological, auger2020introduction}. These challenges make the MCMC approach
unfeasible in fitting SSMs for ecological data assimilation problems.
Alternative methods such as SMC methods have been
explored in literature.

The SMC methods provide a convenient simulation-based approach to
approximate the posterior distributions of the latent states \citep{doucet2001introduction}. They estimate filtering distributions using
sequential importance sampling and when new data is obtained, the
particles are updated via the same sequential importance sampling given
the new data \citep{doucet2001introduction, michaud2021sequential}.
That is, the SMC algorithm iteratively re-samples particles based on their
weights, propagating them forward in time using the state transition
model and then updating their weights based on the likelihood of the
observations. The various SMC methods explored in the literature include
bootstrap filters \citep{gordon1993novel}, auxiliary particle filters \citep{pitt1999filtering}, Lui-West particle filters \citep{liu2001combined}, ensemble Kalman filter \citep{evensen2003ensemble}, particle learning \citep{carvalho2010particle}, etc. These algorithms vary in the importance sampler and resampler schedule used \citep{newman2023state}. To make model fitting easier for ecologists, R packages such as nimbleSMC \citep{michaud2021sequential}, rbiips \citep{todeschini2014biips} and rbi \citep{murray2013bayesian} have been developed that implement some SMC algorithms (see \citet{newman2023state} for a review of packages for various SMC algorithms).

The SMC methods mentioned in the previous paragraph assume that all
parameters in the SSM are constant. In most ecological problems, other
stochastic SSM parameters such as covariate effects would be of
interest. Recent developments such as particle MCMC (pMCMC) \citep[pMCMC; ][]{andrieu2010particle} allow the joint sampling from the posterior
distribution of the latent states and model parameters \citep{andrieu2010particle, gao2012sequential, michaud2021sequential}. The pMCMC puts the SMC algorithms into the
MCMC approaches by replacing the likelihood function with an SMC approximation when sampling from the posterior distribution of the parameters using MMC \citep{newman2023state}, and it can be very sensitive to the parameterisation of the SSM \citep{andrieu2010particle, peters2010ecological}. Moreover, the joint likelihood surfaces of the SSMs can be multimodal \citep{polansky2009likelihood} and non-negligible posterior correlations occur at
high-dimensional parameter space \citep{peters2010ecological}. This leads
to poor convergence and may be slow since they can be stuck at certain
modes of the likelihood function. Coupled with the increase in data
size and potential computational expensiveness of the SSM, pMCMC can also
be computationally unfeasible to re-fit the SSMs once new streams of
data are obtained.

Various suggestions have been made for modelling ecological data that is
sequentially generated such as fitting independent models each time new
data is obtained \citep{kery2020applied}. Although it may
be fast to fit the independent species distribution models, this approach fails to capture the temporal autocorrelation in the data and
can lead to biased inferences on state variables of interest such as
abundance and occupancy. The biased inference of state variables happens because the independent model requires $T$ intercepts (where $T$ is the number of years) and produced a model that is highly overparameterised \citep{kery2020applied}. Therefore, better options for handling this
problem needed to be explored.

Apart from SSMs, ecological time series data can be modelled by defining models that account for the temporal variation in the data as a random effect \citep[for example, year-stratified N-Mixture model; ][]{kery2020applied} or by using conventional time series models like the autoregressive and moving average models \citep{kong2021spatial}. These models can also be fitted in the Bayesian framework by using the standard R packages such as BUGS \citep{lunn2000winbugs, lunn2009bugs}, JAGS \citep{depaoli2016just}, Stan \citep{carpenter2017stan}, NIMBLE \citep{de2017programming}. These models can also be computationally expensive, particularly for over-parameterised models, making it unfeasible to re-fit these over-parameterised models when data are assimilated.

In this study, we propose a modelling framework that
sequentially updates latent state and model parameters
distribution using the posterior model parameters and latent state distribution from an already fitted model. Our proposed framework assumes that an SSM has already been
fitted with MCMC or pMCMC on the old data we had, and we have saved the
posterior samples of the latent states and model parameters. When new
data are received, we use pMCMC to approximate the latent state
distribution at the current time step and also update the posterior
distribution of the model parameters. To achieve this objective, we
modify the particle filtering algorithms (specifically the bootstrap and
auxiliary particle filters) and MCMC samplers from the nimbleSMC package \citep{michaud2021sequential} to a) store the necessary information at
time \(t\) that will be needed to update parameters when new data is
obtained after time step \(t\); b) estimate and update the posterior
distributions of the latent states and model parameters for the new
time steps using the stored information in a). This approach, we think, can relatively reduce the
computational expensiveness and run time of the SSMs. We assess the
performance of our proposed approach to the conventional SMC and MCMC methods
with simulated and real-world data on \textit{Lasius niger} from
\textbf{which survey?} by comparing the effective sample sizes, running
time and Monte Carlo standard errors.


the bias and MCSE from the full model fitted with pMCMC using the auxiliary particle filter were relatively higher than the other full, reduced and updated models. Moreover, there were significant differences between the estimates of $a$ from the reduced model and updated models as $t_r$ increased, but that of $c$ was relatively similar except for $t_r = 20$. Specifically, there 

there was a negative bias in model parameters $a$ and $c$ from both baseline models (BMC, BBSC and ABSC), but a negative bias from BBSC and ABSC and a positive bias from BMC, as observed from Figures \ref{lgssm}; S3-1. As $t_r$ increased, the bias in the model parameters estimated using MCMC (BRMC and ARMC) shrunk towards zero, but that of SMC showed inconsistent patterns. However, the  bias of $a$ and $c$ was closer to zero, but that of $b$ was far from $0$ under all the UMs and for all $t_r$ (Figures \ref{lgssm}; S3-1). 

The MCSE of the model parameters was larger in the baseline and reduced SSMs than the updated models for all $t_r$. As $t_r$ increased, the MCSE of the RM fitted with MCMC (BRMC and ARMC) decreased, as was expected; however, there were inconsistent patterns from the RMs fitted with SMC algorithms (Figures \ref{lgssm}; S3-1). Moreover, as $t_r$ increased, the average root mean squared error of the latent state decreased (Figures \ref{lgssm}; S3-1). However, the precision of the root mean squared error for the SMC models decreased as $t_r$ increased. This suggests that the updated models provided unbiased estimates of the true model parameters, with the mean of the posterior samples of the model parameters being stable and accurate \citep{kruschke2014doing}.

Figure \ref{fig-psifs} shows the estimated annual realised occupancy from the 300 sites, Table \ref{tbl-example2} shows the time taken to run the models fitted to the simulated data, Figure \ref{fig-essEffPlotEx2} shows the effective sample size and efficiency of proposed MCMC sampler for the model parameters, Table S3-1 shows the estimated model parameters from the study models  and Figures S3-5 to S3-6 displays the MCMC convergence plots.

Irrespective of the number of particles (M) used for the SMC models, the updated models simulated more presences than there should be but still captured the trend of the occupied sites for the last ten years (Figure \ref{fig-psifs}). This behaviour of the updated models was no different from baseline SMC models (ABSC and BBSC), suggesting that the overestimation of the occupied sites was related to the sequential Monte Carlo method and not the number of particles. Although the true occupied sites were overestimated by the updated models, the bias in the model parameters was similar to the reduced and baseline models fitted with MCMC, although the precision was lower for the updated models (Table S3-1). 

\begin{longtable}[]{@{}cc@{}}
\caption{\label{tbl-example2}Time taken to fit the dynamic occupancy model using the various approached described in Table \ref{table:modelSummary}.}\tabularnewline
\toprule()
Model  & Times run (minutes)  \\
\midrule()
\endfirsthead
\toprule()
Model &Times run (minutes) \\
\midrule()
\endhead
BMC &  295 \\
RMC &  247 \\
BUMC & 2724 \\
AUMC &  143 \\

\bottomrule()
\end{longtable}



(although the trend looks static from 2019 to 2013 for BUMC, the estimates follow the trajectory of BMC but estimates are closer to the previous year estimates). 

Both BMC and BUMC had similar trajectories for the autoregressive year effect and annual realised occupancy throughout the study period. This high variability and imprecision of the estimates during those years were due to the small sample sizes. Although there was high variability in the BMC for the first 19 years, the variability of the realised occupancy probability was stable for both models, except for the estimates from 2019 to 2023 where the precision of BMC was higher than that of BUMC.

Figure \ref{fig-example4} further showed a decrease in the occupancy probability of Black garden ants in the first ten years (1970 - 1980) of the study, an increase in occupancy probability for the next 18 years (1980 - 1998), followed by a decline in occupancy probability for another ten years (1999 - 2010). For the next 12 years (2011 - 2022), there was an increase in the occupancy probability of Black garden ants, but in 2023 the occupancy probability was very low. 

Two typical questions naturally arise from implementing this updated model framework. The first question involves how long a time series data should be to fit the RMs and UMs. The answer to this question, unfortunately, is not a cast-in-stone one. The simulation studies (sections \ref{simulation-study-one} and \ref{simulation-study-two}) revealed that the updated models performed better relative to the performance of the reduced models. Furthermore, the results from example 1 elaborated that as time $t_r$ increased, the bias and Monte Carlo standard error of model parameters as well as the root mean square error of the latent state reduced (Figure \ref{lgssm}, Supplementary Information 3 Figure 1). With a simple linear Gaussian SSM, it is easy to note that the reduced model moved closer to the true parameter values even for $t_r = 5$, but this may not be the case for more complex SSMs as described in examples 2 - 4 which are data hungry. We suggest that priority should be placed on obtaining better model fits for the reduced model, as is done for most predictive models where the best predictive model is needed to obtain better predictions on new data [REF].


Consistently throughout these three models, the derived quantities from the UMs were highly variable and imprecise. This can be attributed to the smaller sample sizes that were used to fit the updated models.

Although particle MCMC was used in this study, we are sceptical if other SMC algorithms like the Lui-West filters \citep{liu2001combined} and iterated filtering algorithms \citep{ionides2006inference} that simulate the latent state and model parameters together can yield any improvement in model efficiency, an observation noted by \cite{knape2012fitting} and \cite{newman2023state}. However, we propose the use of the Hamiltonian Monte Carlo approach \citep{neal2011mcmc} that updates both model parameters and latent states \citep{newman2023state} can be explored to properly capture the model parameter space. 


Furthermore, the particle MCMC implemented by R-package \textit{nimbleMCMC} \citep{michaud2021sequential} samples all the model parameters from a random walk block sampler. This sampler is very efficient for smaller dimensions of the model parameters \citep{tibbits2014automated}, as can be observed from the trace plots in Supplementary Information 3. For higher dimensions, the pMCMC exhibits stickiness where the model parameters get stuck at some proposed values \citep{michaud2021sequential}. Moreover, the model parameters included variance parameters that were positive and covariate effects that could take on any real number. This leads to different distributional choices for the model parameters, which also leads to the stickiness of the pMCMC chains (see trace plots for simulation study 2 and case study one; Figures S3.5-6). This stickiness can potentially be dealt with by increasing the number of particles \citep{michaud2021sequential}.

 
 
 , we used the mean bias, average root mean square error and Monte Carlo standard error (MCSE) as our model performance metrics (section \ref{simulation-study-one}). In the second simulation, we examined trends of functions of the latent state (section \ref{simulation-study-two}), the behaviour of the chains and the performance of the proposed samplers by estimating the effective sample size and efficiency (i.e., the number of independent samples per unit time) from the chains of the updated SSMs.
 
 Furthermore, the realised or finite sample occupancy, defined as $ psi.fs = \frac{\sum_{i = 1}^N z_{it}}{N}$, where $N$ is the number of sites, is monitored to assess the trend over time \citep{royle2007bayesian}.

 \begin{figure}[htbp!]
\centering 
\includegraphics{Figures/psifs.png}
\caption{\label{fig-psifs} Annual realised occupancy probability estimated from the dynamic occupancy model fitted to the simulated data up to time $t=55$ years using MCMC (BMC), dynamic occupancy model fitted to the simulated data up to time $t=45$ years using MCMC (RMC) and the updated RMC model using pMCMC with auxiliary particle filter (AUMC) and bootstrap particle filter (BUMC) for the simulated data (simulation study two; section \ref{simulation-study-two}). The realised occupancy probability was calculated as the average latent state ($z$) realisations per year. The true realised occupancy probability (labelled truth) is coloured in black, and the time $t$ used to fit the reduced model is indicated by the red vertical line. The correlation between the true realised occupancy probability and the estimated realised occupancy probability from the full model using MCMC is denoted as $R^2_{1}$; the correlation between the true realised occupancy probability and the estimated realised occupancy probability from the reduced model for the first $45$ years using MCMC is denoted as $R^2_{2}$; the correlation between the true realised occupancy probability and the estimated realised occupancy probability from the updated model (BUMC) is denoted as $R^2_{3}$; and the correlation between the true realised occupancy probability and the estimated realised occupancy probability from the updated model (AUMC) is denoted as $R^2_{4}$.}
\end{figure}

For the first $45$ years, all the models estimated the trend of the true realised occupancy probability well (Figure \ref{fig-psifs}). For the last $10$ years, the estimates of the realised occupancy probability from the updated models were higher than those from the full model and the true values. However, the correlation between the occupancy probabilities estimated from the updated models and the true values was $0.99$. This indicated that the trend of the occupancy probability for the last $10$ years was captured by the updated models.

The full model took about five hours to run, the reduced dynamic occupancy model took about four hours to run, the updated dynamic occupancy model fitted using the auxiliary particle filter took about two and half hours to run, and the updated dynamic occupancy model fitted using the bootstrap particle filter took over $47$ hours to run. Although the computational times differed for the various models, the model parameter estimates from all of them were similar (Table S3-1), and all MCMC chains seemed to converge (Supplementary Information Three Figure 3 - 5). Furthermore, the number of independent samples of the model parameters over the run time was higher for the updated model fitted using the pMCMC with an auxiliary particle filter. However, all the approaches generated similar independent samples (Figure \ref{fig-essEffPlotEx2}). This meant that the gain of using our proposed modelling framework for data assimilation problems is its efficiency in generating independent samples.

\begin{figure}[htbp!]
\centering 
\includegraphics{Figures/essEffPlotEx2.png}
\caption{\label{fig-essEffPlotEx2} First column: Effective sample size (ESS) of model parameters estimated from dynamic occupancy model fitted with MCMC to the observed data up to time $55$ (BMC), reduced dynamic occupancy model fitted using MCMC to the observed data up to $t=45$ years (RMC) and updated dynamic occupancy models fitted using bootstrap and auxiliary particle filters (BUMC and AUMC respectively). Second column: Efficiency of model parameters estimated from the full model (BMC), reduced model (RMC) and updated models (BUMC and AUMC). The models were fitted using $M = 50$ particles.}
\end{figure}

and the percentage annual growth rate is estimated as:






We present the correlation of the realised occupancy probability  for years $t+1$ to $20$ between its estimates from the fitted models and the true values from the simulated data and bias of   from all the fitted models in Figure \ref{fig-psifs}. The realised occupancy probability is estimated as follows:
\begin{equation}
    \psi^{fs}_t = \frac{\sum_{i = 1}^N z_{it}}{N},
\end{equation}
where $N$ is the number of sites, and the percentage annual growth rate is estimated as:
\begin{equation}
    \text{Growth rate} = \bigg( \bigg(\frac{\psi^{fs}_{20}}{\psi^{fs}_1}\bigg)^{1/20} -1   \bigg) \times 100.
\end{equation}
Moreover, the computational times of each algorithm used to fit the dynamic occupancy model are presented in Table \ref{tab-computationaltime}. The estimates of the model parameters are presented in Supplementary Information Three Table 1. The effective sample size and efficiency of some selected model parameters and the MCMC convergence checks of the fitted models are presented in Supplementary Information Three Figures 4 -8.


 The distribution of the model parameters is comparable between the updated models (BUMC and AUMC). However, there was no difference in the estimates of the model parameters $a$ and $c$ from the reduced and updated models. Furthermore, the bias in the model parameters estimated from all the models fitted reduced as $t$ approached to $T$. Although estimates were similar in the reduced and updated models, the MCSE of the samples are smaller in updated models than in the reduced model (RMC), and when $t = 49$, the updated models have smaller MCSE than the full models.

\begin{figure}[ht!]
\centering 
\includegraphics{Figures/example2.png}
\caption{\label{fig-example3} Mean population size and growth rate of the Swiss Crested Tit, estimated from full (BMC), reduced (RMC) and updated (BUMC and AUMC) demographic state-space models. The reduced model was fitted to data from 1999 to 2011 and the reduced models were updated using the data from 2012 to 2016. The width of the interval around the posterior mean shows the standard deviation of the estimates, and the vertical line (in red) shows the year $t$ that was used to fit the reduced model. }
\end{figure}


 \subsubsection{Effect of $M$ and $t$}
In simulation study one, we kept the number of particles ($M$) constant and varied the number of years used to fit the reduced model ($t$) (section \ref{simulation-study-one}), but in simulation study two, we varied both $M$ and $t$ (section \ref{simulation-study-two}). 

 The trajectory of the population size and interannual growth rate obtained from BMC was similar to the results in Figure 1.13 in \cite{kery2020applied}.

 However, the estimated population size from the full model was higher than that of the reduced and updated models between 1996 and 2011. The estimates of the population size and interannual growth rate from the updated models were very high, even though we set an upper bound for the latent abundance $N$. We tried various upper bound values to check the estimates stability. However, the population size and growth rate estimates were overestimated in all these instances. 

The reduced model took $20$ minutes to run, the full model took $34$ minutes to run, and the updated models (AUMC and BUMC) took $11$ and $88$ minutes respectively to run. In other words, if we ran the reduced model and then wanted to update our inferences after we obtained new data (the full model) it would take a total of 54 minutes to run, whereas if we updated the reduced model using the auxiliary particle filter (AUMC) it would take a total of 31 minutes to run. This further illustrates the computational gain in updating the existing or reduced model with our proposed framework. Moreover, these differences could quickly add up when running models for many species, as is often done for biodiversity analyses and indicators.


an upper bound was set for the population size, and informative priors were provided for the occupancy models' latent true presence and absence state. 


higher dimensions where the model parameters get stuck at some proposed values \citep{michaud2021sequential}. In this study, we proposed one random walk block sampler for the top-level model parameters and another random walk block sampler for the intermediary model parameters. 

There are various MCMC algorithms that can be used for the pMCMC, and different problems may require different sampling algorithms to efficiently generate samples. The interest is in obtaining proposal methods that use the marginal likelihood approximated with the SMC method. 




The studies further revealed that the results from the models fitted using the auxiliary and bootstrap particle filters are similar .



Our approach thus presents a feasible alternative that can be used for a wide range of monitoring projects, making it much easier to update regular (e.g. annual) reports of the state of nature. , and this objective is well suited to our proposed modelling framework. This study used one ant species: Black Garden Ant, but the framework can be generalised across many species, as well as to multispecies occupancy models.



The proposed framework capitalises on the strength of importance sampling to update model parameters and the latent state distribution of a state space model. Using the saved posterior distribution of the model parameters and latent state from the model fitted using MCMC, the model parameters and latent state distribution were sequentially updated by using particle MCMC \citep{andrieu2010particle}. This updating process was implemented by changing the bootstrap and auxiliary particle filter algorithms in the \textit{nimbleSMC} R-package \citep{michaud2021sequential}.



Typically, the Markovian structure of SSMs allows latent states distribution at time $t$ to be updated by using state processes at time $t-1$ and $t$  and observed data at time $t$ only, whilst the model parameters would need all the observed data \citep{newman2023state}. Depending on the dimension of the model parameters and latent states, SSMs can be computationally expensive (or slower) \citep{newman2023state}, making it unfeasible to refit them to update model parameters and the latent state distribution whenever new data is obtained. For example, the SSMs fitted using the updated method with auxiliary particle filter used 50\% of the time taken by the full models to fit the simulated data in the second simulation study (section \ref{simulation-study-two}), and about 35\% of the minutes used by the full or baseline method respectively to fit the demographic SSM described in section \ref{case-study-two}. This makes the proposed framework computationally feasible for data assimilation problems. Indeed, with increasingly large datasets and increasingly complex models (REF), run times can become a bottleneck for biodiversity analyses (REF). Thus, the reduction in run times achieved by the proposed framework  has great potential for future biodiversity analyses.

In addition to the time taken to fit the SSMs, the proposed framework captured the true model parameters as well as the baseline and reduced method did (and in some instances better as shown in example 1; Figures \ref{lgssm}, Supplementary Information 3 Table 3). The distribution of the model parameters from the updated method moved around the distribution from the reduced methods because we chose the proposal distribution for the model parameters to be $\pi(\theta^{\star}|\theta_r)$ and when $\theta^{\star}$ is rejected, we choose $\theta^{\star}= \theta_r$. In some instances, the updated models explored the parameter space to move closer to the true values of the model parameters better than the reduced models. 

 Simulation study two and case study two showed that the updated method captured the trend in realised occupancy estimated by the baseline method. However, the estimated realised occupancy was either lower or higher than the full model (Figures \ref{fig-psifs} and \ref{fig-example3}). A similar assertion cannot be made in the trend of population size and growth rate of the Swiss Created Tits that were fitted with demographic SSM (Figure \ref{example4}). Generally, Binomial N-Mixture models are known to have unstable parameter estimates, as the model parameter estimates are sensitive to the choice of the upper bound \citep{knape2018sensitivity, dennis2015computational}. Our proposed method yielded unstable estimates of population size and inter-annual growth rate, although we assigned an upper bound for the population size.

A relevant question related to implementing our proposed framework deals with the information that must be stored. Ideally, the posterior distribution of all model parameters, other stochastic nodes, and the latent state distribution at time $t_r$ (see equation \ref{framework}) should be stored. In practice, however, this would require more infrastructure to maintain the stored information over the long term. Alternatively, fewer samples of the model parameters, other stochastic nodes and the latent state distribution are saved for future use. If fewer samples are saved, we can draw more samples from the posterior distribution and use this information to update the existing model. 





 Theory shows that the quality of the likelihood approximation affects how the chain mixes and the efficiency of the pMCMC \citep{andrieu2015convergence, andrieu2016establishing, fearnhead2018particle}. The theory further shows that increasing the number of particles improves the mixing of the pMCMC, and that as the number of observations increases, one needs to increase the number of particles linearly to achieve a good level of mixing \citep{fearnhead2018particle}. However, increasing the number of particles increases the computational expense of the pMCMC \citep{michaud2021sequential, fearnhead2018particle}, especially for higher dimensional latent state space, and this can make the proposed approach challenging to use for some SSMs. Hence, the number of particles chosen to fit SSMs using the updating approach must be carefully chosen to obtain efficiency in the updated methods.

 \begin{figure}
\centering 
\includegraphics{Figures/spartaPsifs.png}
\caption{\label{fig-example4} First row: yearly autoregressive effect accounting for the temporal variation in the data estimated from the full or baseline model (BMC), reduced model (RMC) and updated model (AUMC). Second row: annual realised occupancy (psi.fs) estimated from the full or baseline model (BMC), reduced model (RMC) and updated model (AUMC). The dashed vertical line denotes the year used to fit the reduced model ($2018$).}
\end{figure}

Furthermore, complex SSM structures can pose problems for model validation and assessment \citep{auger2021guide}. Also, the joint likelihood surfaces of such SSMs can be multimodal \citep{polansky2009likelihood}, and non-negligible posterior correlations occur at high-dimensional parameter space \citep{peters2010ecological}. This can lead to poor/slow convergence since the algorithm can become stuck at certain modes of the likelihood function  \citep{andrieu2010particle, peters2010ecological},  \citep{wang2007latent, peters2010ecological, auger2020introduction}.  

However, the estimates from these algorithms were different from those from \textit{sparta}. There are a few reasons for that. \textit{sparta} uses the Gibbs sampling algorithms in JAGS to fit the model, however, the full model fitted with \textit{nimble} assigns various sampling algorithms (we use the default samplers assigned by the NIMBLE platform) to draw from the posterior distribution of the model parameters and latent states.  The reduced model was fit using different default samplers assigned to the model when fitted using \textit{nimble}. As was mentioned in section \ref{model-set-up}, we only sample the latent state values for sites where there was no detection for the full model using \textit{nimble} and our proposed algorithm, but \textit{sparta} draws samples for all sites whether there was a detection or not. These differences in sampling algorithms and simulation of latent states make it difficult for us to make a direct comparison between the results from the full model fitted with \textit{sparta} and our proposed algorithm.

\begin{equation}\label{Growthrate}
\begin{split}
 \text{Correlation($\Psi$)} &= corr(\hat{\Psi}_{t+1:T}^{fs}, {\Psi}_{t+1:T}^{fs})\\
    \text{Bias($\Psi$)} &= \bigg[ \bigg(\frac{\hat{\Psi}^{fs}_{T}}{\hat{\Psi}^{fs}_1}\bigg)^{1/T} -  \bigg(\frac{\Psi^{fs}_{T}}{\Psi^{fs}_1}\bigg)^{1/T}  \bigg] \times 100,\\
\end{split}
\end{equation}

In the vignette attached as Supplementary Information 4, we show how to update models fitted using JAGS with our proposed algorithm.

A closer observation revealed that the estimated realised occupancy from both the full and reduced model for the first year was $1$, and this means that the growth rate would depend on how well the full and updated models estimated the realised occupancy probability at the last year ($T=20$).


Equation \ref{weights} implies that 

The draws of the latent states from the posterior distribution of the reduced model $\{{x}^{(i)}_{1:t}\}_{i = 1}^{N}$ are assumed to be equally weighted. Hence, for all-time steps $1, 2, \ldots, t$ and for all \(M\) particles, the importance weights of these samples ($\{x^{(i)}_{1:t}\}_{i = 1}^{N}$) are assumed to be \(1/M\). Thus, the distribution of the latent states $\text{x}_{1:t}$ is the same for both the reduced and updated models. Then, from time steps \(t +1\) to \(T\), the importance weights are estimated from a chosen particle filter algorithm (for example, bootstrap or auxiliary particle filter).

In summary, for the $i^{th}$ ($i = 1, 2, \ldots, N$) draw of $x_{1:t}$ from the posterior distribution of the reduced model, the following information is used for the particle algorithms in the updating process: 
\begin{equation}\label{weights} 
\left\{
\begin{array}{lll}
      w_t^{(j)} = 1/M & x_{t}^{(j)} = x_{t}^{(i)} & \text{for } 1, 2, \ldots, t \text{ and } 1\leq  j \leq M\\
      w_t^{(j)} \text{ defined by any SMC algorithm }  & x_{t}^{(j)} \text{ from SMC}& \text{for } t+1, t+2, \ldots, T \text{ and } 1\leq  j \leq M\\
\end{array} 
\right. 
\end{equation} 
where $w_t^{(j)}$ is the importance weight for the $j^{th}$ particle and $x_{t}^{(j)}$ is the latent state distribution for $j = 1, 2, \ldots, M$ particles. 

Equation \ref{weights} indicates that each draw of the latent states for time steps $1, 2, \ldots, t$ from the reduced model are replicated $M$ times into the particle filter. For time steps $t+1, 2, \ldots, T$, we simulate $x_{t}^{(j)}$ from its prior distribution and re-sample the $M$ particles using the importance weights $w_t$.
